DARM: Control-Flow Melding for SIMT Thread Divergence Reduction -- Extended Version

GPGPUs use the Single-Instruction-Multiple-Thread (SIMT) execution model where a group of threads-wavefront or warp-execute instructions in lockstep. When threads in a group encounter a branching instruction, not all threads in the group take the same path, a phenomenon known as control-flow divergence. The control-flow divergence causes performance degradation because both paths of the branch must be executed one after the other. Prior research has primarily addressed this issue through architectural modifications. We observe that certain GPGPU kernels with control-flow divergence have similar control-flow structures with similar instructions on both sides of a branch. This structure can be exploited to reduce control-flow divergence by melding the two sides of the branch allowing threads to reconverge early, reducing divergence. In this work, we present DARM, a compiler analysis and transformation framework that can meld divergent control-flow structures with similar instruction sequences. We show that DARM can reduce the performance degradation from control-flow divergence.

==> ae.tex <==
\appendixname{Artifact Appendix}
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}
This artifact contains the source code, python, shell scripts and instructions on how to run the experiments.
This artifact is expected to reproduce the main results in our paper (Figure~\ref{fig:real_benchmark}, \ref{fig:alu_util}, \ref{fig:mem_util}, \ref{fig:profit} and Table~\ref{tab:compile-time}).

Note that the artifact description given below assumes a machine with a {\em Radeon RX Vega 64} GPU with {\em ROCm-4.0.0}. However for the evaluation of our paper we used a newer machine with a {\em Radeon Pro VII} GPU with {\em ROCm-4.2.0}. Unfortunately, this latter machine is not available for remote access, so we provide artifact reviewers remote access to the first machine.

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Algorithm: } Branch Fusion~\cite{branch_fusion}, \name
  \item {\bf Program: } HIP and C/C++ code
  \item {\bf Compilation: } We use {\em gcc-7.5.0} to compile \name compiler. We use {\em hipcc-4.0.20496-4f163c68} to compile the benchmark programs. 
  \item {\bf Binary: } HIP executables
  \item {\bf Data set: } Benchmark programs are either taken form Rodinia~\cite{rodinia}, GPGPU-sim~\cite{ispass2009gpgpusim}, CUDA-Samples~\cite{cu_samples}, GPU-quicksort~\cite{gpu_quicksort_cederman} suites or manually implemented.
  \item {\bf Run-time environment: } {\em Ubuntu 18.04.5 LTS} with {\em ROCm-4.0.0} installed.
  \item {\bf Hardware: } ROCm-compatible GPU. We have tested our approach on AMD {\em Radeon RX Vega 64} and {\em Radeon Pro VII} GPUs. 
  \item {\bf Output: } Speedups, ALU utilization, memory instruction counters, compilation times across benchmarks written into text files.
  \item {\bf Experiment workflow} Download source code and benchmarks, compile the source code, run script to generate the results.
  \item {\bf How much disk space required (approximately)?: } approximately 3.5 GB
  \item {\bf How much time is needed to prepare workflow (approximately)?: } approximately 2 hours
  \item {\bf How much time is needed to complete experiments (approximately)?: } approximately 4 hours
  \item {\bf Publicly available?: } Yes
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{Hardware dependencies}
Our approach requires a GPU that is compatible with {\em ROCm}~\cite{HIPCC} compiler SDK and runtime. We provide artifact reviewers remote access to a machine with an AMD {\em Radeon RX Vega 64} GPU. We expect the reviewer to have a Unix-like environment in order to connect to our remote machine.

To connect to this machine run the following command on an {\em ssh} installed machine. Use the username and password provided by the authors.
\begin{lstlisting}[language=bash, numbers=none]
  $ ssh <username>@tgrogers-pc05.ecn.purdue.edu
\end{lstlisting}
\subsubsection{Software dependencies}
Our approach requires {\em ROCm-4.0.0} driver and compiler SDK installed in the target machine. We use {gcc-7.5.0} and {cmake-3.21.4} for compilation of our source code. To generate the results and plots we use {\em Python 3.6.9} with {\em numpy, pandas, scipy, matplotlib} packages installed. Note that we have pre-installed all these software in our machine, so the reviewers are not required to install them again. 
\subsubsection{Datasets} 
All benchmarks we used are either publicly available or manual reference implementations. For the convenience of the reviewers we provide a repository with all the benchmarks that are ready to use. For benchmark inputs we use randomly generated data (with fixed random seed) with benchmark provided arguments.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Source code}
Our source code and benchmarks repositories are hosted in following {\em gitub} repositories.

  \url{https://github.com/charitha22/cgo22ae-darm-code.git}

  \url{https://github.com/charitha22/cgo22ae-darm-benchmarks.git}


\subsection{Installation}
\noindent
\textbf{Important} : For the subsequent sections including this, please do not copy commands from the PDF. Instead, copy the commands from the README file available at following URL.

\url{https://github.com/charitha22/cgo22ae-darm-benchmarks}

Connect to the remote machine using provide IP address, username and password. Download and build the source code using following set of commands. 
\begin{lstlisting}[language=bash, numbers=none]
  $ export AE_HOME=$(pwd)
  $ git clone https://github.com/charitha22/cgo22ae-darm-code.git
  $ cd cgo22ae-darm-code && mkdir build build_install 
  $ export DARM_HOME=$(pwd)/build
  $ . scripts/run_cmake.sh && make -j4
\end{lstlisting}
This compilation process will take approximately 1 hour. Make sure you use the same shell terminal to execute all the commands/scripts to preserve environment variables. Continue to use the same terminal when running evaluation scripts in the next section.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected result}
Download the benchmarks and evaluation scripts using,
\begin{lstlisting}[language=bash, numbers=none]
  $ cd ${AE_HOME} && git clone https://github.com/charitha22/cgo22ae-darm-benchmarks.git
  $ cd cgo22ae-darm-benchmarks && export BENCH_HOME=$(pwd)
\end{lstlisting}

To generate the speedups plot (Figure~\ref{fig:real_benchmark}) run following commands,
\begin{lstlisting}[language=bash, numbers=none]
  $ . scripts/run_speedups.sh
  $ . scripts/gen_speedups_plot.sh
\end{lstlisting}
Note that {\em speedups.pdf} is generated based on the current experiment results and {\em speedups\_paper.pdf} is generated from the raw numbers used for our paper. 


To generate the ALU utilization plot (Figure~\ref{fig:alu_util}) and memory instruction counters plot (Figure~\ref{fig:mem_util}) use the following commands,
\begin{lstlisting}[language=bash, numbers=none]
  $ . scripts/run_alu_memory_numbers.sh
  $ . scripts/gen_alu_mem_plot.sh
\end{lstlisting}
{\em alu.pdf} and {\em mem.pdf} are generated based on current experiment results and {\em alu\_paper.pdf} and {\em mem\_paper.pdf} are generated using raw numbers used in the paper.

Following commands can be used to generate the melding profitability threshold plot (Figure~\ref{fig:profit}).
\begin{lstlisting}[language=bash, numbers=none]
  $ . scripts/run_profitability_threshold.sh
  $ . scripts/gen_profit_plot.sh
\end{lstlisting}
Similar to above, {\em profitability.pdf} is generated based on current experiment results and {\em profitability\_paper.pdf} is generated based on raw numbers.

Run following commands to obtain the compile times of benchmarks (Table~\ref{tab:compile-time}).
\begin{lstlisting}[language=bash, numbers=none]
  $ . scripts/run_compile_times.sh
  $ . scripts/print_compile_times.sh
\end{lstlisting}
This will print out the compile times for \name and baseline into the standard output.

You can use {\em scp} from your local machine to download the PDF files to your local machine.
\begin{lstlisting}[language=bash, numbers=none]
  $ scp <username>@tgrogers-pc05.ecn.purdue.edu:<location_of_pdf_file> .
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization and reusability}
\subsubsection{Using our method on a new GPU kernel} 
Our compiler can be used on any GPU kernel written in {\em HIP} language. The following commands can be used to compile a GPU kernel with our transformation enabled.
\begin{lstlisting}[language=bash, numbers=none]
  $ mkdir -p tmp
  $ hipcc -### -O3   <kernel_name>.cpp -o <executable_name> 2>&1 | python3 ${DARM_HOME}/../scripts/gen_compile_command.py --llvm-home=/home/cgusthin/workspace/llvm-project-rocm/build \
    --cfmelder-options="" \
    --output-loc=./tmp > ./tmp/compile_command.sh
  $ . ./tmp/compile_command.sh
\end{lstlisting}
These commands automatically generate and runs a sequence of compilation commands that is instrumented with our transformation pass. To demonstrate above compilation process we provide a synthetic {\em HIP} kernel ({\em gpu\_example.cpp}). To compile and run this kernel use the following command.
\begin{lstlisting}[language=bash, numbers=none]
  $ cd ${BENCH_HOME}/customization/gpu_example
  $ make && ./gpu_example
\end{lstlisting}
This kernel contains a divergent {\em if-then-else} branch inside a two-nested loop. {\em If} and {\em then} sections of the branch contain {\em if-then} regions with random computations. This control-flow structure provides multiple melding opportunities for our method. 
You can visualize how \name changed the control-flow of the program using the following commands.
\begin{lstlisting}[language=bash, numbers=none]
  $ ${DARM_HOME}/bin/opt -dot-cfg < ./tmp/gpu_example*.ll > /dev/null
  $ mv .*foo*.dot before.dot
  $ ${DARM_HOME}/bin/opt -dot-cfg < ./tmp/after_pass.ll > /dev/null
  $ mv .*foo*.dot after.dot
\end{lstlisting}
These commands generate {\em .dot} files {\em before.dot} and {\em after.dot} that contains the control-flow graphs of the program before and after the \name transformation. You can view the {\em .dot} files using any online graph viewer\footnote{url{https://dreampuf.github.io/GraphvizOnline/}}.

Our compiler provides several options that can be used to customize the experiments. 
\begin{itemize}[leftmargin=*]
  \item \textbf{--cfmelder-analysis-only} : Only runs the \name analysis (Section~\ref{sec:design:melding_profitability}) and does not modify the program. Analysis can be used to see what parts of the control-flow graph has profitable melding opportunities.
  \item \textbf{--cf-merging-similarity-threshold=$<$threshold$>$} : Adjusts the melding profitability {\em threshold} (Section~\ref{sec:melding_threshold}). {\em threshold} must be a value in the range $[0.0,0.5]$. Setting {\em threshold} to 0.0 will meld any meldable subgraphs (regardless of its profitability), and setting it to 0.5 will only meld subgraphs that are maximally profitable.  
  \item \textbf{--run-cfmelding-on-function=$<$function\_name$>$} : Runs the \name transformation on a specific function only.
  \item \textbf{--run-cfmelding-once} : Disables applying melding recursively. When this option is enabled transformation terminates after performing only one melding.
\end{itemize}
You modify the \textbf{--cfmelder-options} field in the compilation compilation command above to use any of these options.
For example, following modified command will on meld control-flow subgrpahs only if they are maximally profitable (\ie {\em threshold} is 0.5). 
\begin{lstlisting}[language=bash, numbers=none]
  $ mkdir -p tmp
  $ hipcc -### -O3   <kernel_name>.cpp -o <executable_name> 2>&1 | python3 ${DARM_HOME}/../scripts/gen_compile_command.py --llvm-home=/home/cgusthin/workspace/llvm-project-rocm/build \
    --cfmelder-options="--cf-merging-similarity-threshold=0.5" \
    --output-loc=./tmp > ./tmp/compile_command.sh
  $ . ./tmp/compile_command.sh
\end{lstlisting}
You can also update the \textbf{--cfmelder-options} field in the provided {\em Makefile} to achieve the same.

\subsubsection{Using our method on a CPU program}
\name is implemented a general compiler transformation pass and integrated with {\em LLVM opt}. Therefore it can be used on CPU programs as well. To demonstrate this we provide a synthetic program written in {\em C}. Run compile this program run,
\begin{lstlisting}[language=bash, numbers=none]
  $ cd ${BENCH_HOME}/customization/cpu_example
  $ make
\end{lstlisting}
This will generate {\em LLVM-IR} files {\em cpu\_example.input.ll} and {\em cpu\_example.output.ll} that contains the program before and after applying \name transformation. To visualize the control-flow graphs of the two programs run,
\begin{lstlisting}[language=bash, numbers=none]
  $ make dot_cfg
\end{lstlisting}
This will create two {\em .dot} files {\em before.dot} and {\em after.dot} that contains the control-flow graph structure of the original and transformed program. You can copy the content of the {\em .dot} files into an online graph visualizer to view them.

Following command will run the original and transformed programs using {\em LLVM-lli} and also prints the output of the two programs to {\em stdout}.
\begin{lstlisting}[language=bash, numbers=none]
  $ make test
\end{lstlisting}

You can customize {\em cpu\_example.c} to inspect how \name transformation works on different contorl-flow graphs. For example, you can comment out lines $11-14$ and $23-27$ to get a program with different control-flow structure and use above commands to transform and run the programs.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}
\subsubsection{Performance deviation in NQU benchmark } 
We observed that \name does not improve performance in NQU benchmark in the experimental setting provided to the artifact reviewers. 
We attribute this performance deviation to the different {\em LLVM} versions used in {\em rocm-4.0.0} and {\em rocm-4.2.0}. 
The input control-flow graphs provided to \name are different in the two versions and no profitable melding opportunities are available for \name in the case {\em rocm-4.0.0}. Therefore \name does not change the program resulting in identical performance to the baseline and branch fusion. However, with {\em rocm-4.2.0} (which we used for the evaluation of paper) \name does get opportunities for melding and therefore improves the performance. We are unable to change the {\em LLVM} or {\em rocm} version used in the machine because it requires updates to kernel modules and drivers. We provide raw numbers along with scripts to generate the plots used in the paper.

\subsubsection{Limitations of \name implementation}
Current implementation of \name requires that any basic block inside a meldable divergent region (Section~\ref{def:meld_div_region}) $R$ is post-dominted by $R$'s exit block. Therefore basic blocks inside $R$ can not contain {\em return} statements. In addition current implementation of \name does not officially support unstructured control-flow. 
{\em single basic blocks, if-then region, if-then-else regions } and {\em structured loops} or any nesting of these structures are allowed inside a meldable divergent region.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
